UniFashion: A Unified Vision-Language Model for Multimodal Fashion Retrieval and Generation

The fashion domain encompasses a variety of real-world multimodal tasks, including multimodal retrieval and multimodal generation. The rapid advancements in artificial intelligence generated content, particularly in technologies like large language models for text generation and diffusion models for visual generation, have sparked widespread research interest in applying these multimodal models in the fashion domain. However, tasks involving embeddings, such as image-to-text or text-to-image retrieval, have been largely overlooked from this perspective due to the diverse nature of the multimodal fashion domain. And current research on multi-task single models lack focus on image generation. In this work, we present UniFashion, a unified framework that simultaneously tackles the challenges of multimodal generation and retrieval tasks within the fashion domain, integrating image generation with retrieval tasks and text generation tasks. UniFashion unifies embedding and generative tasks by integrating a diffusion model and LLM, enabling controllable and high-fidelity generation. Our model significantly outperforms previous single-task state-of-the-art models across diverse fashion tasks, and can be readily adapted to manage complex vision-language tasks. This work demonstrates the potential learning synergy between multimodal generation and retrieval, offering a promising direction for future research in the fashion domain. The source code is available at https://github.com/xiangyu-mm/UniFashion.

==> Contents/Background.tex <==
\section{Preliminaries}

\subsection{Diverse Fashion Tasks}
Diverse fashion tasks encompass a range of image and language manipulations, including cross-modal retrieval, composed image retrieval, fashion image captioning and generation, etc. 
As shown in Fig.~\ref{FashionTask}, each task uniquely transforms an input model into a specific target model. 
The representative tasks can be briefly divided into the following two groups. 

\noindent \textbf{Representative Fashion Retrieval} generally consists of text-to-image (T2I), image-to-text (I2T) and composed image retrieval (CIR) tasks. 

\noindent \textit{T2I and I2T} tasks are to find the corresponding text or image from a large image corpus $\mathcal{D}$ given an input (either an image or text). 

\noindent \textit{CIR} task is to retrieve a target image from a vast image database based on a reference image and a text description detailing changes to be applied to the reference image. In this scenario, a query pair $p = \{I_{R}, t\}$ is provided, where $I_{R}$ is the reference image and $t$ is the text describing the desired modifications. The challenge for \modelname{} is to accurately identify the target image $I_{T}$ that best matches the query among all potential candidates in the image corpus $\mathcal{D}$.

\noindent \textbf{Representative Fashion Generation} consists of Fashion Image Captioning (FIC) and Fashion Image Generation (FIG). 

\noindent \textit{FIC} aims to generate a descriptive caption for a product based on the visual and/or textual information provided in the input. 

\noindent \textit{FIG} task involves two modes of generating a new image. The first one is Text-to-Image Generation, which generates a fashion image based on an input text description. The other one is Composed Image Generation, which employs visual information and accompanying text instructions as inputs to generate fashion images.

\subsection{Problem Formulation}

Existing fashion image retrieval and generation methods are typically designed for specific tasks, which inherently restricts their applicability to tasks with different target domains. 
Taking the image retrieval model as an example, they accept the caption as input and retrieve the target image as output:
\begin{equation}
    I_{out} = \mathcal{F}_{\mathcal{T}_{Ret}}(C_{in};\Theta),
\end{equation}
where $\mathcal{F}_{\mathcal{T}_{Ret}}$ represents the retrieval model parameterized by $\Theta$. These models can accommodate retrieval tasks, such as image-to-text, text-to-image retrieval. However, these models cannot be extended to perform tasks like image captioning or image generation, which necessitates a completely different output modality.

To train a unified model that can handle multiple fashion tasks, our approach introduces a versatile framework capable of handling multiple fashion tasks by aligning the multimodal representation model into the LLM and the diffusion model. This innovative strategy enhances the model's adaptability, and it can be represented as:
\begin{equation}
    I_{out},T_{out} = \mathcal{F}_{\mathcal{T}_{Ret}, \mathcal{T}_{Gen}}(I_{in}, T_{in}; \Theta),
    \label{single_task}
\end{equation}
where $\mathcal{F}_{\mathcal{T}}$ represents the unified model parameterized by $\Theta$, it consists of retrieval module ${\mathcal{T}_{Ret}}$ and generative module ${\mathcal{T}_{Gen}}$.
